Guided Synthesis of Labeled Brain MRI Data Using Latent Diffusion Models for Segmentation of Enlarged Ventricles

Deep learning models in medical contexts face challenges like data scarcity, inhomogeneity, and privacy concerns. This study focuses on improving ventricular segmentation in brain MRI images using synthetic data. We employed two latent diffusion models (LDMs): a mask generator trained using 10,000 masks, and a corresponding SPADE image generator optimized using 6,881 scans to create an MRI conditioned on a 3D brain mask. Conditioning the mask generator on ventricular volume in combination with classifier-free guidance enabled the control of the ventricular volume distribution of the generated synthetic images. Next, the performance of the synthetic data was tested using three nnU-Net segmentation models trained on a real, augmented and entirely synthetic data, respectively. The resulting models were tested on a completely independent hold-out dataset of patients with enlarged ventricles, with manual delineation of the ventricles used as ground truth. The model trained on real data showed a mean absolute error (MAE) of 9.09 \pm 12.18 mL in predicted ventricular volume, while the models trained on synthetic and augmented data showed MAEs of 7.52 \pm 4.81 mL and 6.23 \pm 4.33 mL, respectively. Both the synthetic and augmented model also outperformed the state-of-the-art model SynthSeg, which due to limited performance in cases of large ventricular volumes, showed an MAE of 7.73 \pm 12.12 mL with a factor of 3 higher standard deviation. The model trained on augmented data showed the highest Dice score of 0.892 \pm 0.05, slightly outperforming SynthSeg and on par with the model trained on real data. The synthetic model performed similar to SynthSeg. In summary, we provide evidence that guided synthesis of labeled brain MRI data using LDMs improves the segmentation of enlarged ventricles and outperforms existing state-of-the-art segmentation models.

==> paper/chapters/abstract.tex <==
Deep learning models in medical contexts face challenges like data scarcity, inhomogeneity, and privacy concerns. Synthetic data can help, but often underperforms compared to real data. This study focuses on improving ventricular segmentation in brain Magnetic Resoncance Imaging (MRI) images, particularly for cases with enlarged ventricles, using synthetic data.
We employed two latent diffusion models (LDMs): a mask generator trained using 10,000 masks, and a corresponding SPADE image generator optimized using 6,881 scans to create an MRI conditioned on a 3D brain mask. Conditioning the mask generator on ventricular volume in combination with classifier-free guidance enabled the control of the ventricular volume distribution of the generated synthetic images. Next, the performance of the synthetic data was tested using three nnU-Net segmentation models trained on a real (N=1,000), augmented (N=1,512) and entirely synthetic data (N=1,000), respectively, where the synthetic data contains a more uniform distribution of ventricular volumes compared to the real data. The resulting models were tested on a completely independent hold-out dataset of patients with enlarged ventricles (N=42), with manual delineation of the ventricles used as ground truth performed by a trained neuroradiologist. The model trained on real data showed a mean absolute error (MAE) of $9.09\pm12.18$ mL in predicted ventricular volume, while the models trained on synthetic and augmented data showed MAEs of $7.52\pm4.81$ mL and $6.23\pm4.33$ mL, respectively. Both the synthetic and augmented model also outperformed the state-of-the-art model SynthSeg, which due to limited performance in cases of large ventricular volumes, showed an MAE of $7.73\pm12.12$ mL with a factor of 3 higher standard deviation. The model trained on augmented data showed the highest Dice score of $0.892\pm0.05$, slightly outperforming SynthSeg ($0.874\pm0.06$) and on par with the model trained on real data ($0.891\pm0.05$). The synthetic model ($0.872\pm0.06$) performed similar to SynthSeg. In summary, we provide evidence that guided synthesis of labeled brain MRI data using LDMs improves the segmentation of enlarged ventricles and outperforms existing state-of-the-art segmentation models. 




%Structure:  
%introduction, methods, results, discussion}

==> paper/chapters/introduction.tex <==
The success of machine learning largely depends on the quantity and quality of available training data. As models grow increasingly large, they require immense datasets, which has culminated in some of the most successful models trained on so many instances of data they need not see the same sample twice (\cite{brown2020language_gpt3}). While such abundance can be found in natural images or natural language processing tasks, this wealth of data is not universally accessible. In medical imaging, data scarcity, variability, and privacy constraints present significant challenges to building similarly large models.

Patients with normal pressure hydrocephalus (NPH) exemplify this issue, displaying an abnormal buildup of cerebrospinal fluid in the brain's ventricle system, consequently leading to unique and abnormally enlarged ventricles. Contemporary state-of-the-art models for brain segmentation of magnetic resonance imaging (MRI) data \cite{billot_robust_synthseg_2023} struggle to accurately segment the enlarged ventricle systems of NPH patients. Furthermore, obtaining a large training set for these patients is difficult due to their uniqueness and the diverse nature of the disease.

Generating synthetic data offers a promising alternative to the prohibitively costly process of collecting real data. Modern image generation models, such as diffusion models, initially seem to provide limitless, highly customizable data with perceptual quality nearly indistinguishable from real images \cite{podell2023sdxl}. However, extensive research has shown that purely synthetic training data cannot match the effectiveness of real training data \cite{marwood2023diversity_diffusion,Fernandez_2022_trained_with_fully_synthetic_data,Fernandez_2024_SyntheticData}. Instead, synthetic data is best used to supplement real data to enhance model performance \cite{azizi2023synthetic_improves_imagnet}. 

In the field of MRI, several studies \cite{pinaya2022brain_image_generation_w_LDM, han2023medgen3d} have demonstrated the remarkable perceptual quality of synthetic images generated using diffusion models. Although these synthetic images still do not match the quality of real data, \cite{Fernandez_2022_trained_with_fully_synthetic_data} has made significant progress in narrowing the performance gap between real and synthetic training data for brain MRI segmentation models. Additionally, conditioning the models on scalar values can produce increasingly realistic and morphology-preserving images. For example, \cite{pinaya2022brain_image_generation_w_LDM} trained a latent diffusion model (LDM) on a large sample of 3D T1-weighted MRI data (N=31,740) from the UK Biobank dataset \cite{Sudlow2015_UK_Biobank} while conditioning on several parameters such as ventricular volume, thus being able to generate synthetic data with varying ventricle sizes. Achieving remarkable visual quality, \cite{pinaya2022brain_image_generation_w_LDM} used their model to create an open large synthetic dataset consisting of 100,000 synthetic 3D MRI images (LDM100k dataset). 

In this study, we extend prior work by presenting two LDMs: a mask generator and an image generator. Combined, these models create fully synthetic labeled segmentation data for brain MRI. By conditioning our mask generator on ventricular volume, we enable control over the distribution in the generated data. We generate synthetic images and labels with out-of-distribution (OOD) ventricle sizes using our LDMs to address data scarcity for patients with enlarged ventricles. Finally, we train a ventricle segmentation model using this synthetic data and compare the performance against state-of-the-art models, using a completely independent test set consisting of NPH patients with enlarged ventricles.

\setcounter{footnote}{0}
Code to reproduce this work is publicly available on GitHub.\footnote{See \url{https://github.com/vaynonym/diffusion_abnormal_brain_anatomy}}

==> paper/chapters/methods.tex <==
\subsection{Data}

\newcommand{\Dldm}{LDM100k Dataset}
\newcommand{\Dflair}{MS-FLAIR Dataset}

\subsubsection{\Dldm}\label{DLM_dataset_definition}

%With real medical data being subject to restrictions in where and how it may be used, the use of synthetic data offers several tempting advantages. Furthermore, as synthetic data has reached a level of quality where it can be used to train models successfully on some downstream tasks \cite{Fernandez_2022_trained_with_fully_synthetic_data}, it can be a viable option to explore further. 

\cite{pinaya2022brain_image_generation_w_LDM} generated a publicly available\footnote{Data can be downloaded from \url{https://academictorrents.com/details/63aeb864bbe2115ded0aa0d7d36334c026f0660b}} large synthetic dataset of 100,000 3D T1-weighted brain MRI images using an LDM trained on UK biobank data \cite{Sudlow2015_UK_Biobank} with isotropic $1$ mm$^3$ voxel size and a resolution of $160$ x $224$ x $160$. In this work, to reduce computational constraints, we first downsampled the data to a spacing of $1.67$ x $1.75$ x $1.67$ $mm^3$ and center-cropped to a resolution of $96$ x $128$ x $96$. We also only used the first 10,000 images in the data to keep the size in line with our other dataset (\Dflair{}), assuming a valid representation of the full dataset. The main purpose of this dataset is two-fold, 1) serving as the training data for our mask diffusion model due to its balanced spread of ventricular volumes, and 2) also being used for transfer learning. To generate segmentation labels for the data, we used the SynthSeg model \cite{billot_robust_synthseg_2023}. In addition to the segmentation, the model also estimates the size of the volumes for different parts of the brain. To obtain the conditioning value $c$, we divided the ventricular volume by the intracranial volume to get the relative size of the ventricles. We subsequently normalized these values between 0 and 1 over the subset of the data, and the outcome was then parsed into the models for conditioning. Lastly, we used a randomized 80-20 schema, splitting the data into training and hold-out validation datasets.

\subsubsection{MS-FLAIR Dataset}

The dataset consists of T2-weighted 3D FLAIR images acquired at the Copenhagen University Hospital - Rigshospitalet, Copenhagen, Denmark. The data comprises 2,927 patients with multiple sclerosis (MS) who were scanned multiple times as part of their treatment, resulting in a total of 6,881 scans. A more thorough description of the data is available at \cite{hindsholm_scanner_2023}. All patient-specific data was handled in compliance with the Danish data protection agency act no. 502. The collection of the retrospective dataset was approved by the National Committee on Health Research Ethics (protocol number 2117506). 

We performed the same steps as for the LDM100k data to obtain segmentation masks and corresponding volumetric estimates for each MRI. Since the LDM100k dataset was spatially aligned, we further cropped the MS-FLAIR dataset placing the brain in the center of the image using the segmentation masks, before downsampling to the same spacing and cropping to the same image size of $96$ x $128$ x $96$.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.98\linewidth]{paper/images/methods/histogram_diffusion_v2.png}
    \caption{Histogram of the distribution of normalized ventricular volumes for the LDM100k data (N=10,000) and the MS-FLAIR data (N=6,881). The x-axis displays the normalized volume ratio $c$, which is estimated as the ratio of ventricular volume to intracranial volume to get the relative size of the ventricles, and subsequently normalized over the data to the range between 0 and 1.}
    \label{fig:dataset_ventricular_volume_comparison}
\end{figure}



A comparison of the distribution of images with respect to ventricular volume can be seen in \autoref{fig:dataset_ventricular_volume_comparison}. It is evident that the \Dflair{} is much less uniformly distributed with respect to ventricular volume than the \Dldm. 

\subsection{Diffusion Models}
\input{paper/chapters/background}

\subsection{Mask Generator Latent Diffusion Model}

In this work, the first step in our model development pipeline to generate synthetic labeled data is to generate masks. For this, we used a diffusion model, specifically an LDM  \cite{rombach2022_highresolution_LDM_synthesis} due to the large computational requirements imposed by working in the 3D image space. The autoencoder architecture and hyperparameters were based on \cite{pinaya2022brain_image_generation_w_LDM}, but given the different target of mask reconstruction instead of images, we made several changes based on an informal hyperparameter search. First, our reconstruction loss consisted of a cross-entropy loss. As labels cannot be trivially used with common perceptual losses and we found no benefit in using an adverserial loss, we used no other additional loss to train the model except for KL-regularization to a normal distribution with a weight of $1\mathrm{e}{-6}$. Next, instead of feeding the labels directly to the model, we used an embedding layer, trained end-to-end, before the first layer, with a feature dimension of 64. We trained the autoencoder for 40 epochs using the \Dldm. For the diffusion model, we followed the basic denoising model and training algorithm from \cite{DDPM}. The backbone of the noise-prediction model was a U-Net with an additional attention mechanism closely resembling \cite{pinaya2022brain_image_generation_w_LDM}. We used conditioning on the normalized ventricular volume ratio $c \in [0, 1]$ (see \autoref{DLM_dataset_definition}) via attention. Further, we used classifier-free guidance \cite{ho2022ClassifierFreeGuidance} by training the model on the conditional and unconditional case at the same time, adding an additional binary conditioning parameter and randomizing $c$ in the unconditional case. The extra parameter was needed to ensure $c$ maintained a smooth distribution which the model can learn more easily. During training, there was a 20\% chance for any dataset entry to be transformed to the unconditional case. The diffusion model was trained for 5 epochs. The low number of epochs was motivated by \cite{dar2024unconditional_memorize_patient_data}, who found that longer training times are associated with reproducing patient data and thus less diversity. For more details, please see \autoref{fig:mask_generator_overview}.

\subsection{Image Generator Latent Diffusion Model}

Now having defined a mask generation LDM (previous subsection), we used the output of that model to condition the image generation (Figure \ref{fig:data_generation_inference_architecture}), following the same general 3D LDM approach.
Specifically, we used a KL-autoencoder similar to the Mask Generator case, but the decoder used the segmentation mask like a SPADE model \cite{park2019_Spade} to enable precise alignment of images with the mask. We used a similar loss combination as in \cite{pinaya2022brain_image_generation_w_LDM}, using a combination of perceptual loss, adverserial loss, pixel-based L1 loss, and KL-loss as in the mask generator case. For the adverserial loss, we used a patch-based discriminator based on \cite{wang2018highresolution_patch_discriminator_basis}. We trained the autoencoder on the \Dldm{} for 20 epochs first to utilize the large and diverse dataset, and then fine-tuned the autoencoder for another 10 epochs on the \Dflair, since the test set used for the downstream segmentation task was acquired using the T2-weighted FLAIR sequence. The diffusion model closely matched the mask generator model architecture. Like the decoder of the autoencoder, the upsampling part of the U-Net backbone also employed SPADE connections. We trained the diffusion model for 20 epochs using the \Dldm{} and fine-tuned for 5 epochs on the \Dflair. 
For an overview of the general training architecture, please see \autoref{fig:Spade_model_architecture}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.97\linewidth]{paper/images/methods/architecture/model_v2.png}
    \caption{Overview of the pipeline used to generate synthetic labeled data. Latent diffusion models (DM) are employed in two stages to produce synthetic brain images and corresponding masks. The pipeline begins with a noise input passed through a Mask DM that can be conditioned on the parameter $c$ reflecting the normalized ventricular volume ratio, followed by denoising to produce a latent representation. A Mask Decoder transforms this latent representation into a synthetic segmentation mask. Parallel to this, a SPADE DM, conditioned on the synthetic mask, generates denoised latent representations which are decoded to create a synthetic brain image. }
    \label{fig:data_generation_inference_architecture}
\end{figure}





==> paper/chapters/related_work.tex <==
Diffusion models have enjoyed increasing attention and success in both research and real-world applications. While first suggested by \cite{original_diffusion_paper}, it was not until \cite{DDPM} significantly simplified and improved the concept that diffusion models took off. Since then, the variational score-based perspective approaching diffusion models with stochastic differential equations has opened the path to improvements to sampling time (\cite{song2022DDIM} \todo{cite more}), while LDMs \cite{rombach2022_highresolution_LDM_synthesis} opened the path to generating high resolution images more efficiently. \cite{park2019_Spade} displayed a new normalization technique that allows efficient conditioning on semantic masks to generate matching images. Models like \cite{podell2023sdxl} have even gained considerable attention beyond academia.

Using diffusion models in a medical context for generating 3D MRI data has been a relatively recent development with the increasing perceptual quality of generative models. \cite{pinaya2022brain_image_generation_w_LDM} trained a latent diffusion model on 3D MRI data from the UK Biobank dataset \cite{Sudlow2015_UK_Biobank} while conditioning on several parameters such as ventricular volume. At generation time, this allows some degree of customizability, such as generating large or small ventricles. Achieving remarkable visual quality, they use their model to create an open large synthetic dataset. Common downstream tasks like segmentation necessitate paired labeled data in order to train models, however. Continuing in the domain of brain MRI, \cite{Fernandez_2022_trained_with_fully_synthetic_data} address this by generating paired data using an LDM mask generator and a Spade (\cite{park2019_Spade}) autoencoder to generate synthetic images. Much attention is focused toward the encoder encoding solely the style of the image in the latent space, thus enabling at test-time the generalization to different styles of image domain and datasets. In \cite{Fernandez_2024_SyntheticData}, this approach is extended to 3D. 

While previously noted approaches generate images in one model pass, ~\cite{han2023medgen3d} presents a slice-wise approach toward generating 3D synthetic data with paired masks. Casting the mask generation as a sequential problem conditioned on previously generated slices along with a sophisticated architecture to ensure consistency, their approach manages to handle the great memory constraints imposed by high resolution 3D medical data. This constitutes a possible way to address potential problems we later point out with our simple down-sampling approach.
